Ein Fenster zur gleichzeitigen Messung der Uebertragungsfunktion eines realen Systems und des Leistungsdichtespektrums des ueberlagerten Rauschens am Systemausgang (Teil 2)

The method described in the first part for frequency-selectively measuring the transfer function and the noise power spectral density of the superimposed noise at the output of a disturbed, real system with nonlinearities using windowing was limited to time-invariant systems with stationary and zero-mean processes. Here, we investigate how this measurement method can be extended so that all correlations existing between the input and output signals can also be measured using windowing for a periodically time-varying system disturbed by a cyclostationary noise process. An extended version of the window construction algorithm presented in the first part is introduced, in which some degrees of freedom not used there can be used to appropriately influence the properties of the window sequence depending on the application. -- Das im ersten Teil beschriebene Verfahren die Uebertragungsfunktion und das Rauschleistungsdichtespektrum des ueberlagerten Rauschens am Ausgang eines gestoerten, realen Systems mit Nichtlinearitaeten mit Hilfe der Fensterung frequenzselektiv zu vermessen beschraenkte sich auf zeitinvariante Systeme mit stationaeren und mittelwertfreien Prozessen. Hier wird untersucht, wie dieses Messverfahren zu erweitern ist, so dass man damit auch alle Korrelationen, die zwischen Ein- und Ausgangssignal bestehen, bei einem periodisch zeitvarianten System, das von einem zyklostationaeren Rauschprozess gestoert wird, mit einer Fensterung messen kann. Es wird eine erweiterte Variante des im ersten Teil vorgestellten Algorithmus zur Konstruktion des Fensters angegeben, bei der einige dort nicht genutzte Freiheitsgrade dazu verwendet werden koennen, die Eigenschaften der Fensterfolge je nach Applikation geeignet zu beeinflussen.

==> mbild1d1.tex <==
\put(    120.000000000000,    545.000000000000){\makebox(0,0){\includegraphics[
width=    160.000000000000\unitlength,height=    160.000000000000\unitlength,clip]{pbild1d1.pdf}}}


==> mbild1d10.tex <==
\put(    320.000000000000,     60.000000000000){\makebox(0,0){\includegraphics[
width=    120.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild1d10.pdf}}}


==> mbild1d2.tex <==
\put(    340.000000000000,    535.000000000000){\makebox(0,0){\includegraphics[
width=    120.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild1d2.pdf}}}


==> mbild1d3.tex <==
\put(     60.000000000000,    365.000000000000){\makebox(0,0){\includegraphics[
width=    120.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild1d3.pdf}}}


==> mbild1d4.tex <==
\put(    200.000000000000,    365.000000000000){\makebox(0,0){\includegraphics[
width=    120.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild1d4.pdf}}}


==> mbild1d5.tex <==
\put(    394.000000000000,    365.000000000000){\makebox(0,0){\includegraphics[
width=    120.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild1d5.pdf}}}


==> mbild1d6.tex <==
\put(     60.000000000000,    218.000000000000){\makebox(0,0){\includegraphics[
width=    120.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild1d6.pdf}}}


==> mbild1d7.tex <==
\put(    200.000000000000,    218.000000000000){\makebox(0,0){\includegraphics[
width=    120.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild1d7.pdf}}}


==> mbild1d8.tex <==
\put(    394.000000000000,    218.000000000000){\makebox(0,0){\includegraphics[
width=    120.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild1d8.pdf}}}


==> mbild1d9.tex <==
\put(    120.000000000000,     60.000000000000){\makebox(0,0){\includegraphics[
width=    120.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild1d9.pdf}}}


==> mbild3b1.tex <==
\put(    200.000000000000,    200.000000000000){\makebox(0,0){\includegraphics[
width=    400.000000000000\unitlength,height=    400.000000000000\unitlength,clip]{pbild3b1.pdf}}}


==> mbild3b10.tex <==
\put(    225.000000000000,    100.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild3b10.pdf}}}


==> mbild3b11.tex <==
\put(    225.000000000000,    100.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild3b11.pdf}}}


==> mbild3b2.tex <==
\put(    110.000000000000,    500.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild3b2.pdf}}}


==> mbild3b3.tex <==
\put(    340.000000000000,    500.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild3b3.pdf}}}


==> mbild3b4.tex <==
\put(    110.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild3b4.pdf}}}


==> mbild3b5.tex <==
\put(    340.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild3b5.pdf}}}


==> mbild3b6.tex <==
\put(    110.000000000000,    500.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild3b6.pdf}}}


==> mbild3b7.tex <==
\put(    340.000000000000,    500.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild3b7.pdf}}}


==> mbild3b8.tex <==
\put(    110.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild3b8.pdf}}}


==> mbild3b9.tex <==
\put(    340.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    220.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild3b9.pdf}}}


==> mbild4f1.tex <==
\put(    125.000000000000,     80.000000000000){\makebox(0,0){\includegraphics[
width=    210.000000000000\unitlength,height=    160.000000000000\unitlength,clip]{pbild4f1.pdf}}}


==> mbild4f2.tex <==
\put(    345.000000000000,     80.000000000000){\makebox(0,0){\includegraphics[
width=    210.000000000000\unitlength,height=    160.000000000000\unitlength,clip]{pbild4f2.pdf}}}


==> mbild4g.tex <==
\put(    225.000000000000,    280.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    600.000000000000\unitlength,clip]{pbild4g.pdf}}}


==> mbild4h.tex <==
\put(    225.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    600.000000000000\unitlength,clip]{pbild4h.pdf}}}


==> mbild4i.tex <==
\put(    225.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    600.000000000000\unitlength,clip]{pbild4i.pdf}}}


==> mbild5c1.tex <==
\put(    225.000000000000,    500.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild5c1.pdf}}}


==> mbild5c2.tex <==
\put(    225.000000000000,    300.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild5c2.pdf}}}


==> mbild5c3.tex <==
\put(    225.000000000000,    100.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    200.000000000000\unitlength,clip]{pbild5c3.pdf}}}


==> mbild5u.tex <==
\put(    225.000000000000,    185.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    370.000000000000\unitlength,clip]{pbild5u.pdf}}}


==> mbild6a1.tex <==
\put(    115.000000000000,    305.000000000000){\makebox(0,0){\includegraphics[
width=    190.000000000000\unitlength,height=    190.000000000000\unitlength,clip]{pbild6a1.pdf}}}


==> mbild6a10.tex <==
\put(    225.000000000000,    190.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    100.000000000000\unitlength,clip]{pbild6a10.pdf}}}


==> mbild6a11.tex <==
\put(    225.000000000000,     50.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    100.000000000000\unitlength,clip]{pbild6a11.pdf}}}


==> mbild6a12.tex <==
\put(    225.000000000000,    490.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild6a12.pdf}}}


==> mbild6a13.tex <==
\put(    225.000000000000,    320.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild6a13.pdf}}}


==> mbild6a14.tex <==
\put(    225.000000000000,    190.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    100.000000000000\unitlength,clip]{pbild6a14.pdf}}}


==> mbild6a15.tex <==
\put(    225.000000000000,     50.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    100.000000000000\unitlength,clip]{pbild6a15.pdf}}}


==> mbild6a16.tex <==
\put(    225.000000000000,    480.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    160.000000000000\unitlength,clip]{pbild6a16.pdf}}}


==> mbild6a17.tex <==
\put(    225.000000000000,    320.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild6a17.pdf}}}


==> mbild6a18.tex <==
\put(    225.000000000000,    190.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    100.000000000000\unitlength,clip]{pbild6a18.pdf}}}


==> mbild6a19.tex <==
\put(    225.000000000000,     50.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    100.000000000000\unitlength,clip]{pbild6a19.pdf}}}


==> mbild6a2.tex <==
\put(    355.000000000000,    305.000000000000){\makebox(0,0){\includegraphics[
width=    190.000000000000\unitlength,height=    190.000000000000\unitlength,clip]{pbild6a2.pdf}}}


==> mbild6a3.tex <==
\put(    225.000000000000,     80.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    160.000000000000\unitlength,clip]{pbild6a3.pdf}}}


==> mbild6a4.tex <==
\put(    225.000000000000,    520.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    120.000000000000\unitlength,clip]{pbild6a4.pdf}}}


==> mbild6a5.tex <==
\put(    225.000000000000,    355.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    130.000000000000\unitlength,clip]{pbild6a5.pdf}}}


==> mbild6a6.tex <==
\put(    225.000000000000,    190.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    140.000000000000\unitlength,clip]{pbild6a6.pdf}}}


==> mbild6a7.tex <==
\put(    225.000000000000,     40.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=     80.000000000000\unitlength,clip]{pbild6a7.pdf}}}


==> mbild6a8.tex <==
\put(    225.000000000000,    495.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    130.000000000000\unitlength,clip]{pbild6a8.pdf}}}


==> mbild6a9.tex <==
\put(    225.000000000000,    335.000000000000){\makebox(0,0){\includegraphics[
width=    450.000000000000\unitlength,height=    130.000000000000\unitlength,clip]{pbild6a9.pdf}}}

